Bridging Dimensions: Confident Reachability for High-Dimensional Controllers

Autonomous systems are increasingly implemented using end-to-end learning-based controllers. Such controllers make decisions that are executed on the real system, with images as one of the primary sensing modalities. Deep neural networks form a fundamental building block of such controllers. Unfortunately, the existing neural-network verification tools do not scale to inputs with thousands of dimensions -- especially when the individual inputs (such as pixels) are devoid of clear physical meaning. This paper takes a step towards connecting exhaustive closed-loop verification with high-dimensional controllers. Our key insight is that the behavior of a high-dimensional controller can be approximated with several low-dimensional controllers. To balance the approximation accuracy and verifiability of our low-dimensional controllers, we leverage the latest verification-aware knowledge distillation. Then, we inflate low-dimensional reachability results with statistical approximation errors, yielding a high-confidence reachability guarantee for the high-dimensional controller. We investigate two inflation techniques -- based on trajectories and control actions -- both of which show convincing performance in three OpenAI gym benchmarks.

==> subsections/HSCC-proof.tex <==
\section{Proof for tube containment problem in the HSCC version}

We define the exact action discrepancy, denoted as $\delta(s)$, as a function that takes a specific state as an input and outputs the L1 distance of the control action difference between HDC and LDC. 
\begin{definition}[Exact action discrepancy function]\label{def:exact-time-discrepancy}
Given any state $s$ within the state space $S$, the exact action-based discrepancy function, denoted as $\delta(s)$, is defined as follows: 
    \begin{align*}
        \delta(s) =  \| \chd(g(s)) - \cld(s) \|_1
    \end{align*}
\end{definition}

With the help of the exact action discrepancy function $\delta$, we can define the $\delta$-based inflated reachable set. This inflated reachable set at time $t$ is inflated on the last inflated reachable set at time $t-1$. Therefore, the recursive form of $\delta$-based inflated reachable set is written as, 
\begin{align*}
    \drs(0) &= S_0, \\
    \drs(1) &= \Bigl\{ f(s,u) \mid s \in \drs(0), 
    u \in [\cld(s) - \delta(s), \cld(s) + \delta(s)] \Bigl\},  \\
    \drs(2) &= \Bigl\{ f(s,u) \mid s \in \drs(1), 
    u \in [\cld(s) - \delta(s), \cld(s) + \delta(s)] \Bigl\},\\
    \cdots\\
    \drs(t) &= \Bigl\{ f(s,u) \mid s \in \drs(t-1), 
    u \in [\cld(s) - \delta(s), \cld(s) + \delta(s)] \Bigl\}.
\end{align*}

This recursive formulation allows us to construct the $\delta$-based inflated reachable set over time. We provide the formal definition of this inflated reachable set below.

\begin{definition}[$\delta$-based inflated reachable set]\label{def:drs}
Given the low-dimensional system \mld, the exact action discrepancy function $\delta(s)$, the initial set $S_0$, and the last $\delta$-based inflated reachable set $\drs(t-1)$ propagating from $S_0$, the $\delta$-based inflated reachable set at time $t$ is defined as follows: 
% {\color{blue}will pick up one for better proof in the future}
    \begin{align*}
        \drs(t) = \Bigl\{ f(s,u) \mid s \in \drs(t-1), 
        u \in [\cld(s) - \delta(s), \cld(s) + \delta(s)] \Bigl\}, && \\
        \text{where at time}~t=0,  \drs(0) = S_0. 
    \end{align*}
    
    % \begin{align*}
    %     \drs(t) = \Bigl\{ f(s,u) \mid  s \in \drs(t-1), 
    %     u \in \{ \cld(s) - \delta(s), \cld(s) + \delta(s) \} \Bigl\}, && \\
    %     \text{where at time}~t=0,  \drs(0) = S_0.
    % \end{align*}

    % \begin{align}
    %     \rs_{HDC}(S_{t-1}) = \Bigl\{ f(s,u) \Big|   s \in S_{t-1}, 
    %     u = \chd(g(s)) \Bigl\}.  
    % \end{align}

\end{definition}

Based on Definition 17, the $\delta$-based inflated reachable tube can be defined below.

\begin{definition}[$\delta$-based inflated reachable tube]\label{def:drt}
Given the initial set $S_0$, the exact action discrepancy function $\delta(s)$, and the time horizon $T$, the $\delta$-based inflated reachable tube is defined as a sequence of $\delta$-based inflated reachable sets over time $T$:
    \begin{align*}
        \drt(S_0, T) = [S_0, \drs(1), \cdots, \drs(T-1), \drs(T)].\\
        % \irt_{\mld}(S_0, T, \delta(s)) = [S_0, \irs(S_0, 1, \delta(s)), \irs(S_0, 2, \delta(s)),\\
        % \cdots, \irs(S_0, T-1, \delta(s))  ].
    \end{align*}

\end{definition}

\begin{comment}

Based on Def 3.13, given the exact action-based discrepancy function $\delta$, the recursive version of the $\delta-based$ inflated reachable tube can be written as:
    \begin{align*}
     \irt(S_0, T, \delta(s)) = [S_0, \irs(S_0, \delta(s)), \irs(\irs(S_0, \delta(s)), \delta(s)),\\
        \irs(\irs(\irs(S_0, \delta(s)), \delta(s)), \delta(s)), \cdots, \irs \underbrace{( \cdots(\irs(S_0, \delta(s)), \cdots, \delta(s))}_\text{T-1}, \delta(s)) ].
    \end{align*}

To simplify the format of $\delta-based$ reachable tube, we make $\irs(S_0, t, \delta(s))$ represent $\delta-based$ inflated reachable set at time $t$: 
    \begin{align*}
    \irs(S_0, t, \delta(s)) = \irs\underbrace{( \cdots(\irs(S_0, \delta(s)), \cdots, \delta(s))}_\text{t-1}, \delta(s)),\\ \text{where at time 0 } \irs(S_0, 0, \delta(s)) = S_0.
    \end{align*}



\begin{definition}[$\delta-\textit{based}$ inflated reachable tube]
Given the initial set $S_0$, the exact action-discrepancy function $\delta(s)$, and the time horizon $T$,
    \begin{align*}
        \irt_{\mld}(S_0, T, \delta(s)) = [S_0, \irs(S_0, 1, \delta(s)), \irs(S_0, 2, \delta(s)),\\
        \cdots, \irs(S_0, T-1, \delta(s))  ].
    \end{align*}
    % \begin{align*}
    %     \irt_{\mld}(S_0, T, \delta(s)) = \{S_0, \irs(S_0, 1, \delta(s)), \irs(\irs(S_0, 1, \delta(s)), 2, \delta(s)), \\
    %     \irs(\irs(S_0, 2, \delta(s)), 3, \delta(s)), \cdots, \irs(\irs(S_0, T-1, \delta(s)), T ,\delta(s))   \}
    % \end{align*}

    % \begin{align*}
    %     \irt_{\mld}(S_0, T, \delta(s)) = \{S_0, \irs(S_0, \delta(s)), \irs(\irs(S_0, \delta(s)), \delta(s)), \\
    %     \irs(\irs(\irs(S_0, \delta(s), \delta(s)), \delta(s)), \cdots, \irs( \cdots \irs(S_0, \delta(s)), ,\delta(s))   \}
    % \end{align*}

\end{definition}

\end{comment}

Following a similar procedure, we define the high-dimensional reachable set and tube in the expression of low-dimensional space below. 

\textcolor{blue}{This HDC reachable set definition expresses the same meaning as definitions 2 and 3. The reason I want to redefine is to keep the consistency for all the definitions of set and tube, which can be easy to prove our lemma. Will choose one later.}
\begin{definition}[High-dimensional reachable set]\label{def:hds}
Given the high-dimensional system \mhd, the initial set $S_0$, the current time $t$, and the last high-dimensional reachable set $\rs_{\mhd}(t-1)$ propagating from $S_0$, the high-dimensional reachable set at time $t$ is defined as: 
    \begin{align*}
        \rs_{\mhd}(t) = \Bigl\{ f(s,u) \mid s \in \rs_{\mhd}(t-1), 
        u = \chd(g(s)) \Bigl\}, && \\
        \text{where at time}~t=0,  \rs_{\mhd}(0) = S_0. 
    \end{align*}

\end{definition}

\begin{definition}[High-dimensional reachable tube]\label{def:hdt}
Given the initial set $S_0$, the time horizon $T$, the high-dimensional reachable tube is defined as a sequence of high-dimensional reachable sets over time $T$:
    \begin{align*}
        \rt_{\mhd}(S_0, T) = [S_0, \rs_{\mhd}(1), \cdots, \rs_{\mhd}(T-1), \rs_{\mhd}(T)].\\
        % \irt_{\mld}(S_0, T, \delta(s)) = [S_0, \irs(S_0, 1, \delta(s)), \irs(S_0, 2, \delta(s)),\\
        % \cdots, \irs(S_0, T-1, \delta(s))  ].
    \end{align*}

\end{definition}



Therefore, with the help of Definition~\ref{def:drt} and ~\ref{def:hdt}, we get our lemma~\ref{lemma: HDCcontainment} showing that the $\delta$-based inflated reachable tube contains the high-dimensional reachable tube.

\begin{lemma}\label{lemma: HDCcontainment}
    Consider the high-dimensional system \mhd and the low-dimensional system \mld, both starting from the same initial set $S_0$. Let us calculate the high-dimensional reachable tube $\rt_{\mhd}(S_0, T)$ and the $\delta$-based reachable tube $\drt(S_0, T)$ over the same time horizon $T$. The $\drt(S_0, T)$ contains the $\rt_{\mhd}(S_0, T)$: $$\rt_{\mhd}(S_0, T) \subseteq \drt(S_0, T).$$
\end{lemma}

 
\begin{proof}
To prove lemma \ref{lemma: HDCcontainment}, we need to prove that 
\begin{align}\label{eq:lemma2-hd-contain}
\forall t \in \{1,..., T\}, \rs_{\mhd}(t) \subseteq \drs(t).
\end{align}

Base case: From Definitions~\ref{def:drs} and~\ref{def:hds}, the two reachable sets at time $t=1$ can be written as,
\begin{align}
        \drs(1) &= \Bigl\{ f(s,u) \mid s \in S_0, 
        u \in [\cld(s) - \delta(s), \cld(s) + \delta(s)] \Bigl\}\\
        \rs_{\mhd}(1) &= \Bigl\{ f(s,u) \mid s \in S_0, 
        u = \chd(g(s)) \Bigl\}
\end{align}
Based on the Definition \ref{def:exact-time-discrepancy}, the $\delta$-based control action set to calculate $\drs(1)$ contains the exact high-dimensional control action set to calculate $\rs_{\mhd}(1)$. Also, both of them start from the same initial set $S_0$. So, we conclude that $\rs_{\mhd}(1) \subseteq \drs(1)$. Note that these two sets can be equal when the HDC and LDC have zero control action difference for every state inside the set $S_0$.

Induction phase: Assume the $\rs_{\mhd}(t) \subseteq \drs(t)$, the statement $\rs_{\mhd}(t+1) \subseteq \drs(t+1)$ should also hold. At time $t+1$, the two reachable sets can be expressed as, 
\begin{align}
        \drs(t+1) &= \Bigl\{ f(s,u) \mid s \in \drs(t), 
        u \in [\cld(s) - \delta(s), \cld(s) + \delta(s)] \Bigl\}\\
        \rs_{\mhd}(t+1) &= \Bigl\{ f(s,u) \mid s \in \rs_{\mhd}(t), 
        u = \chd(g(s)) \Bigl\}
\end{align}

Given that $\rs_{\mhd}(t) \subseteq \drs(t)$, the $\delta$-based control action set from $\drs(t)$ to calculate $\drs(t+1)$ includes the exact high-dimensional control action set from the $\rs_{\mhd}(t)$ to calculate $\rs_{\mhd}(t)$. In short, both the control action set and the last reachable set in the $\delta$-based approach include the control action set and the last reachable set in the high-dimensional setting. Therefore, $\rs_{\mhd}(t+1) \subseteq \drs(t+1)$. Following the same procedure for each time step in the time horizon $T$, the equation \ref{eq:lemma2-hd-contain} is valid. Therefore, the lemma \ref{lemma: HDCcontainment} holds.

% Next, at time $t=2$, the two reachable sets can also be written as,
% \begin{align}
%         \drs(2) &= \Bigl\{ f(s,u) \mid s \in \drs(1), 
%         u \in [\cld(s) - \delta(s), \cld(s) + \delta(s)] \Bigl\}\\
%         \rs_{\mhd}(2) &= \Bigl\{ f(s,u) \mid s \in \rs_{\mhd}(1), 
%         u = \chd(g(s)) \Bigl\}
% \end{align}

% Since we have already proved that $\rs_{\mhd}(1) \subset \drs(1)$, the control action set to  calculate $\drs(2)$ encompasses the control action set to calculate $\rs_{\mhd}(2)$. We also conclude $\rs_{\mhd}(2) \subset \drs(2)$. Following the same procedure for the time horizon $T$, we can prove equation \ref{eq:lemma2-hd-contain} is valid. Therefore, the lemma \ref{lemma: HDCcontainment} holds.
\end{proof}

However, obtaining the $\delta$-based reachable set is impractical because this involves solving an optimization problem over a complex, high-dimensional space. Also, we cannot examine each state within the state space. Consequently, we opt for an alternative approach by establishing the statistical upper bound for the exact action discrepancy $\delta$, denoted as $\bgamma$ defined below. 

\begin{definition}[\textit{Time-variant statistical action-based discrepancy}]{\label{def:time-variant-gamma}}
Given the HDC \chd, the distilled LDC \cld, a confidence $\alpha \in (0, 1)$, a set $S_t$ that is reachable at time $t$, and any distribution $D_t$ for sampling states over $S_t$, the time-variant statistical action-based discrepancy $\bgamma_{D_t}$ is such that:
\begin{align*}
 \prob_{s \sim D_t}\big( \|\chd(g(s)) - \cld(s)\|_1 \leq \bar{\gamma}_{D_t} \big) \geq 1 - \alpha
\end{align*}
\end{definition}


Drawing from Definition~\ref{def:time-variant-gamma}, we establish the $\gamma$-based time-variant inflated reachable set. In the verification of the LDC, we can determine the set of control actions corresponding to the LDC and the last reachable set. This calculated control action set is expanded by this time-variant statistical action-based discrepancy $\bar{\gamma}$. Subsequently, the $\gamma$-based inflated reachable set is overapproximated with this inflated control action set. Note that the time-variant statistical action-based discrepancy $\bgamma$ is determined by sampling states following some unknown distribution $D$ over the last reachable set.

Given the fact that the next $\gamma$-based inflated reachable set is derived from the last $\gamma$-based reachable set, we adopt the recursive form akin to the $\delta$-based inflated reachable set. The key difference is that we add another argument, namely the distribution for sampling random states in this recursive form. This method defines our $\gamma$-based reachable set below. At the time $t=0$, the initial set is the $S_0$. Our recursive form starts from $t=1$:
\begin{align*}
    \grs(1, D_0) &= \Bigl\{ f(s,u) \mid s \in S_0, 
    u \in [\cld(s) - \bgamma_{D_0}, \cld(s) + \bgamma_{D_0}] \Bigl\}, \\
    \grs(2, D_1, D_0) &= \Bigl\{ f(s,u) \mid s \in \grs(1, D_0), 
    u \in [\cld(s) -\bgamma_{D_1}, \cld(s) + \bgamma_{D_1}] \Bigl\}, \\
    \cdots \\
    \grs(t, D_{t-1}, \cdots, D_0) &= \Bigl\{ f(s,u) \mid s \in \grs(t-1, D_{t-2}, \cdots, D_0), 
    u \in [\cld(s) - \bgamma_{D_{t-1}}, \cld(s) + \bgamma_{D_{t-1}}] \Bigl\}.
\end{align*}


% \begin{definition}[$\gamma$-based time-variant inflated reachable set]
% Given a low-dimensional system \mld, the HDC \chd, the current time $t$, a sequence of distribution $\mathcal{D}_{t-1}$ for sampling states in each time step over the time horizon $t-1$, denoted as $\mathcal{D}_{t-1}= \{ D_i \}_{i=1}^{t-1}$, the last $\gamma$-based reachable set $\grs(t-1, D_{0:t-2})$, where the $D_{0:t-2} \subset \mathcal{D}_{t-1}$, 
% the $\gamma$-based time-variant inflated reachable set at time $t(t\geq 1)$ is defined as:
%     \begin{align*}
%         \grs(t, \mathcal{D}_{t-1}) =   \Bigl\{ f(s,u) \Big|   s \in \grs(t-1, \mathcal{D}_{t-2}), 
%         u \in [\cld(s) - \gamma_{D_{t-1}}, \cld(s) + \gamma_{D_{t-1}} ] \Bigl\}.  
%     \end{align*}  
% \end{definition}


\begin{definition}[$\gamma$-based time-variant inflated reachable set]
Given a low-dimensional system \mld, the HDC \chd, the current time $t$, a sequence of distribution $\mathcal{D}= \{ D_i \}_{i=1}^{t}$, $D_{0:t-1} = \{ D_i \}_{i=1}^{t-1} \subset \mathcal{D}$, the $\gamma$-based time-variant inflated reachable set at time $t(t\geq 1)$ is defined as:
    \begin{align*}
        \grs(t, D_{0:t-1}) =   \Bigl\{ f(s,u) \Big|   s \in \grs(t-1, D_{0:t-2}), 
        u \in [\cld(s) - \gamma_{D_{t-1}}, \cld(s) + \gamma_{D_{t-1}} ] \Bigl\}.  
    \end{align*}
\end{definition}

\begin{definition}[$\gamma$-based time-variant inflated reachable tube]
Given the initial set $S_0$, the low-dimensional system \mld, the HDC \chd, the time horizon $T$, and a sequence of time-variant distributions $\mathcal{D} = \{ D_i \}_{i=1}^{T-1}$, where for the specific time $t$ ($t \leq T$), we denote the corresponding sequence of distribution as $D_{0:t} =  \{ D_i \}_{i=1}^{t}$, the $\gamma$-based time-variant inflated reachable tube is defined as a sequence of reachable sets:
    % \begin{align*}
    %   \grt(S_0, T, \bm{\mathcal{D}}) = [S_0, \grs(1, \mathcal{D}_0), \grs(2, \mathcal{D}_1), \cdots, \grs(t-1, \mathcal{D}_{t-2}), \grs(t, \mathcal{D}_{t-1})]
    % \end{align*}
    \begin{align*}
      \grt(S_0, T, \mathcal{D}) = [S_0, \grs(1, D_0), \grs(2, D_{0:1}), \cdots, \grs(t-1, D_{0:t-2}), \grs(t, D_{0:t-1})]
    \end{align*}
\end{definition}
{\color{blue}{Time-invariant version will be added once I finish the proof of the time-variant version because the time-invariant is weaker due to the fixed sampling distribution over the time $T$}}


% Previous version of  for variant inflated reachable tube]
% Given the initial set $S_0$, the low-dimensional system \mld, the HDC \chd, a sequence of time-variant distribution $\mathcal{D} = \{ D_t \}_{t=1}^{T-1}$ to get a corresponding sequence of statistical action discrepancy $\bar{\bm{{\gamma}}}_\mathcal{D} = \{\bar{\gamma}_{D_i}\}_{i=0}^{T-1}$, and the time horizon $T$, the $\gamma$-based time-variant inflated reachable tube is defined as a sequence of reachable sets:

% \begin{definition}[$\gamma$-based time-variant inflated reachable tube]
% Given the initial set $S_0$, the low-dimensional system \mld, the HDC \chd, a sequence of sets of time-variant distributions $\bm{\mathcal{D}} = \{\mathcal{D}_0, \mathcal{D}_1, \dots, \mathcal{D}_{T-1} \}$ (or $\bm{\mathcal{D}} = \{D_0, D_1, \dots, D_{T-1} \}$ and we denote that $D_{0:t} = \{ D_0, \cdots, D_t \}$) to get a corresponding sequence of $\gamma$-based reachable sets, and the time horizon $T$, the $\gamma$-based time-variant inflated reachable tube is defined as a sequence of reachable sets:
%     \begin{align*}
%       \grt(S_0, T, \bm{\mathcal{D}}) = [S_0, \grs(1, \mathcal{D}_0), \grs(2, \mathcal{D}_1), \cdots, \grs(t-1, \mathcal{D}_{t-2}), \grs(t, \mathcal{D}_{t-1})]
%     \end{align*}
%     \begin{align*}
%       \grt(S_0, T, \bm{\mathcal{D}}) = [S_0, \grs(1, D_0), \grs(2, D_{0:1}), \cdots, \grs(t-1, D_{0:t-2}), \grs(t, D_{0:t-1})]
%     \end{align*}
% \end{definition}
% {\color{blue}{Time-invariant version will be added once I finish the proof of the time-variant version because the time-invariant is weaker due to the fixed sampling distribution over the time $T$}}



\begin{comment}
    
Based on Def 3.16, given the sequence of the time-variant statistical action-based discrepancy $\bar{{\gamma}} = \{\bar{\gamma_{D_i}}\}_{i=0}^{T-1}$, the recursive version of the inflated reachable tube is defined below:
    \begin{align}
     \irt(S_0, T, \bar{\gamma}) = [S_0, \irs(S_0, \bar{\gamma}_{D_0}), \irs(\irs(S_0, \bar{\gamma}_{D_0}), \bar{\gamma}_{D_1}),\\
        \irs(\irs(\irs(S_0, \bar{\gamma}_{D_0}), \bar{\gamma}_{D_1}), \bar{\gamma}_{D_2}), \cdots, \irs \underbrace{( \cdots(\irs(S_0, \bar{\gamma}_{D_0}), \cdots, \bar{\gamma}_{D_{T-2}})}_\text{T-1}, \bar{\gamma}_{D_{T-1}}) ]
    \end{align}
    To simplify this definition of the reachable tube, following a similar procedure of the $\delta-based$ inflated reachable set, we define the $\gamma-based$ inflated reachable set at time $t$: 
    \begin{align*}
    \irs(S_0, t, \bar{\gamma}_{t-1}) = \irs\underbrace{( \cdots(\irs(S_0, \bar{\gamma}_{D_0}), \cdots, \bar{\gamma}_{D_{t-2}})}_\text{t-1}, \bar{\gamma}_{D_{t-1}}),\\ \text{where at time 0 } \irs(S_0, 0, \bar{\gamma}_{D_{-1}}) = S_0.
    \end{align*}

\begin{definition}[$\gamma$-based time-variant inflated reachable tube]
Given the initial set $S_0$, the low-dimensional system \mld, the time-variant statistical action-discrepancy $\bar{\bm{{\gamma}}}_\mathcal{D} = \{\bar{\gamma}_{D_i}\}_{i=0}^{T-1}$, and the time horizon $T$, the $\gamma-\textit{based}$ time-variant inflated reachable tube is such that:
    \begin{align*}
      \irt(S_0, T, \bar{\gamma}) = [S_0, \irs(S_0, 1, \bar{\gamma}_{D_0}), \irs(S_0, 2, \bar{\gamma}_{D_1}), \cdots \irs(S_0, T, \bar{\gamma}_{D_{T-1}})]
    \end{align*}
\end{definition}
\end{comment}

\begin{lemma}\label{lemma:dgtube-contain}
Given the initial set $S_0$, time horizon $T$, the $\mathcal{D}$ represents a sequence of sets of time-variant distributions for sampling states, denoted as $\mathcal{D} = \{ D_i \}_{i=1}^{T-1}$, 
% where the $\mathcal{D}_{t} = \{ D_i\}_{i=1}^{t}$ represents a sequence of distributions for sampling states to obtain the $\grs(t, \mathcal{D}_{t-1})$, 
the $\gamma$-based reachable tube contains the $\delta$-based reachable tube with at least a probability of $(1-\alpha)^T$,

    % \begin{align}\label{def:dgtube-contain}
    % \prob_{\bm{\mathcal{D}}}\Big[\drt(S_0, T) \subseteq \grt(S_0, T, \bm{\mathcal{D}}) \Big] \geq 1-\alpha.
    % \end{align}
    
    \begin{align}\label{def:dgtube-contain2}
\prob_{\mathcal{D}}\Big[\drt(S_0, T) \subseteq \grt(S_0, T, \mathcal{D}) \Big] \geq (1-\alpha)^T.
    \end{align}
\end{lemma}

\begin{proof}
 If we want to prove lemma~\ref{lemma:dgtube-contain}, we need to prove all the $\gamma$-based reachable sets contain all the $\delta$-based reachable sets over the time horizon $T$ with at least $1-\alpha$ probability,
\begin{align}\label{eq:lemma3-onemore}
    \prob_{\mathcal{D}} \big[ \drs(t) \subseteq \grs(t, D_{0:t-1}), \forall t \in \{1, ..., T \}  \big] \geq (1- \alpha)^T
\end{align}
Base phase: I define the events $E_1 = \{\drs(1) \subseteq \grs(1, D_0)\}, E_2 = \{ \drs(2) \subseteq \grs(2, D_{0:1}) \}, \cdots, E_T = \{ \drs(T) \subseteq \grs(T, D_{0:T-1}) \}$. It's straightforward to get the probability of $E_1$, namely $P(E_1) \geq 1 - \alpha$ and straightforward to obtain the probability of $E_2$ given the $E_1$ holds, namely $P(E_2 \mid E_1) \geq 1 - \alpha$. Therefore, the probability of both events happening is that $P(E_2 \cap E_1) = P(E_2 \mid E_1) \times P(E_1) \geq (1 - \alpha)^2$. Then move one more step,  we assert that $P(E_3 \cap E_2 \cap E_1) = P(E_3 \mid E_1 \cap E_2) \times P(E_1 \cap E_2) = (1 - \alpha)^3$

Induction phase: Given the fact based on the conformal prediction that $P(E_T \mid E_1 \cap E_2 \cap ... \cap E_{T-1}) \geq 1-\alpha$  and $P(E_1 \cap E_2 \cap ... \cap E_{T-1}) > (1-\alpha)^{T-1} $, we assert that $P(E_1 \cap E_2 \cap ... \cap E_{T}) =  (E_T \mid E_1 \cap E_2 \cap ... \cap E_{T-1}) \times P(E_1 \cap E_2 \cap ... \cap E_{T-1}) \geq (1-\alpha)^T$. Therefore, the equation \ref{eq:lemma3-onemore} holds and then the Lemma 3 holds.


\end{proof}

\begin{comment}The previous dead-end of the previous lemma 3.
\begin{proof}

A \textit{Counter example} was discovered during the proof. If we want to prove lemma~\ref{lemma:dgtube-contain}, we need to prove all the $\gamma$-based reachable sets contain all the $\delta$-based reachable sets over the time horizon $T$ with at least $1-\alpha$ probability,
\begin{align}
    \prob_{\bm{\mathcal{D}}} \big[ \drs(t) \subseteq \grs(t, \mathcal{D}_{t-1}), \forall t \in \{1, ..., T \}  \big] \geq 1- \alpha
\end{align}

Starting from the distribution $D_0$ over the initial set $S_0$ at time $t=0$, we obtain two control action sets for calculating $\delta-$, $\gamma$-based reachable set:
\begin{align}
    U_{\delta}^0 = \{u| s \in S_0, u \in [\cld(s) - \delta(s), \cld(s) + \delta(s) ]  \} 
    \label{eq:Ut0delta-0}
\end{align}
\begin{align}
U_{\bar{\gamma}_{D_0}}^0 = \{u| s \in S_0, u \in [\cld(s) - \bar{\gamma}_{D_0}, \cld(s) + \bar{\gamma}_{D_0} ]    \} \label{eq:Ut0gamma-0}
\end{align}

Based on lemma~\ref{lemma:org-cp}, Definiton~\ref{def:exact-time-discrepancy},~\ref{def:time-variant-gamma}, and equation~\ref{eq:Ut0delta-0},~\ref{eq:Ut0gamma-0}, we conclude that

\begin{align}
    \prob_{\mathcal{D}_0}\big[U_{\delta}^0 \subseteq U_{\bar{\gamma}_{D_0}}^0 \big] \geq 1 - \alpha \label{eq:deltagammaU-0}
\end{align}

Since our verification guarantees that the next reachable set is calculated by considering all the states in the last set $S_0$ and all the control actions in the set $U_{\delta}^0$ or $U_{\bar{\gamma}}^0$, drawing from equation~\ref{eq:deltagammaU-0}, we conclude that,
\begin{align}\label{eq:1st-step}
    \prob_{\mathcal{D}_0}  \Big[ \drs(1) \subseteq \grs(1, \mathcal{D}_0)\Big] \geq 1-\alpha 
\end{align}

Then, we need to demonstrate that the second $\gamma$-based reachable set contains the second $\delta$-based reachable set still with a probability of at least $1-\alpha$. Following the same procedure, the control action sets for $\gamma-based$ and $\delta-based$ reachable set are denoted as:

\begin{align}
    U_{\delta}^1 = \{u| s \in \drs(1), u \in [\cld(s) - \delta(s), \cld(s) + \delta(s) ]  \} 
    \label{eq:Ut0delta}
\end{align}
\begin{align}
    U_{\bar{\gamma}_{D_1}}^1 = \{u | s \in \grs(1, \mathcal{D}_0), u \in [\cld(s) - \bar{\gamma}_{D_1}, \cld(s) + \bar{\gamma}_{D_1} ]    \} \label{eq:Ut0gamma}
\end{align}

Given that the set $\grs(1, \mathcal{D}_0)$, applied to calculate the $\bgamma_{D_1}$, differs from the set $\drs(1)$, employed to calculate the next $\delta$-based reachable set, we cannot assure any guarantee of the action difference in the second step. Therefore, $\prob_{\mathcal{D}_1}[U_{\delta}^1 \subseteq U_{\bar{\gamma}_{D_1}}^1 ]$ is unknown. Furthermore, $\prob_{\mathcal{D}_1}  \Big[ \drs(2) \subseteq \grs(2, \mathcal{D}_1)\Big]$ remains undetermined.
{\color{blue} Maybe have a chance to get the probability by considering the conditional probability.}
% Since the set $\grs(1)$ for sampling states to calculate the $\bar{\gamma}_{D_1}$ is not the same as $\drs(1)$ that is used to calculate the next $\delta$-based reachable set. The guarantee of difference between control actions doesn't hold in the second step, namely $\prob_{s \sim D_1}(U_{\delta}^1 \subseteq U_{\bar{\gamma}}^1 )$ is unknown.
\end{proof}
\end{comment}

\subsection{Mixed tube approach (incomplete)}

But this is a pretty loose bound unless we set the error rate to be pretty tiny such as 0.001, which is impractical in the implementation. So, we put forward the $\gamma-\delta$ mixed inflated reachable set. This reachable set still originates from the same initial set $S_0$ and this reachable set at $t=1$ is the $\delta$-based reachable set at $t=1$, denoted as $\mrs(1) = \drs(1)$. However, starting from the time $t=2$, the mixed $\gamma-\delta$ reachable set was inflated on the last $\gamma$-based inflated reachable set with the exact action discrepancy $\delta$. The recursive form of this mixed $\gamma-\delta$ reachable set starting from $t=2$ is denoted as:

\begin{align*}
    \mrs(2, D_0) &= \Bigl\{ f(s,u) \mid s \in \grs(1, D_0), 
    u \in [\cld(s) -\delta(s), \cld(s) + \delta(s)] \Bigl\},\\ 
    \mrs(3, D_{0:1}) &= \Bigl\{ f(s,u) \mid s \in \grs(2, D_{0:1}), 
    u \in [\cld(s) -\delta(s), \cld(s) + \delta(s)] \Bigl\},\\
    \cdots\\
    \mrs(t, D_{0:t-2}) &= \Bigl\{ f(s,u) \mid s \in \grs(t-1, D_{0:t-2}), 
    u \in [\cld(s) - \delta(s), \cld(s) + \delta(s)] \Bigl\}.
\end{align*}


\begin{definition}[$\gamma-\delta$ mixed inflated reachable set]
Given the low-dimensional system \mld, the HDC \chd, and a sequence of sets of distributions $D_{0:t-2} = \{D_i\}_{i=0}^{t-2}$ to obtain the last $\gamma$-based reachable set $\grs(t-1, D_{0:t-2})$, the $\gamma-\delta$ mixed inflated reachable set at time $t (t \geq 2)$ is defined as:
    % \begin{align*}
    %     \mrs(t, \mathcal{D}_{t-2}) =   \Bigl\{ f(s,u) \Big|   s \in \grs(t-1, \mathcal{D}_{t-2}), 
    %     u \in [\cld(s) - \delta(s), \cld(s) + \delta(s) ] \Bigl\}. %\text{where the $\irs(S_0, 0, %\gamma_{-1}) = S_0 $ }  
    % \end{align*}
    \begin{align*}
        \mrs(t, D_{0:t-2}) =   \Bigl\{ f(s,u) \Big|   s \in \grs(t-1, D_{0:t-2}), 
        u \in [\cld(s) - \delta(s), \cld(s) + \delta(s) ] \Bigl\}. %\text{where the $\irs(S_0, 0, %\gamma_{-1}) = S_0 $ }  
    \end{align*}
\end{definition}


\begin{comment}
    
The mixed $\gamma-\delta$ inflated reachable tube is defined as:
    \begin{align*}
     \irt_{mix}(S_0, T, \bar{\gamma}, \delta) = [S_0, \irs(S_0, \delta), \irs(\irs(S_0, \bar{\gamma}_{D_0}), \delta),\\
        \irs(\irs(\irs(S_0, \bar{\gamma}_{D_0}), \bar{\gamma}_{D_1}), \delta), \cdots, \irs \underbrace{( \cdots(\irs(S_0, \bar{\gamma}_{D_0}), \cdots, \bar{\gamma}_{D_{T-2}})}_\text{T-1}, \delta) ]
    \end{align*}

To simplify the expression, 

\begin{align*}
    \irs_{mix}(S_0, t, \bar{\gamma}_{t-1}, \delta) = \irs\underbrace{( \cdots(\irs(S_0, \bar{\gamma}_{D_0}), \cdots, \bar{\gamma}_{D_{t-2}})}_\text{t-1}, \delta), \text{where } t \geq 2.
\end{align*}
\end{comment}

% $\bar{\bm{{\gamma}}}_\mathcal{D} = \{\bar{\gamma}_{D_i}\}_{i=-1}^{T-2}$, the $\gamma-\delta$ 
\begin{definition}[$\gamma-\delta$ mixed inflated reachable tube]
Given the initial set $S_0$, the time horizon $T$, the low-dimensional system \mld, the HDC \chd, and a sequence of time-variant distributions $\mathcal{D} = \{D_0, D_1, \dots, D_{T-2} \}$, where at specific time $t (t\geq 2)$, $D_{0:t} = \{ D_i \}_{i=0}^{t}$, to get a corresponding sequence of $\gamma$-based inflated reachable sets, the $\gamma-\delta$ mixed inflated reachable tube is denoted as a sequence of the $\gamma-\delta$ mixed inflated reachable sets:
    \begin{align*}
      \mrt(S_0, T, \mathcal{D}) = [S_0, \drs(1), \mrs(2, D_{0}), \cdots, \mrs(T, D_{0:T-2})]
    \end{align*}
\end{definition}

\begin{lemma}\label{lemma:mgtube-contain}
Given the system \mld, the HDC \chd,  the initial set $S_0$, time horizon $T$, the $\mathcal{D}$ represents a sequence of time-variant distributions for sampling states over the last-step inflated reachable set, denoted as $\mathcal{D} = \{ D_t \}_{t=1}^{T-1}$, where the $D_t$ represents any distribution for sampling states over the $\grs(S_0, t-1)$, the $\gamma$-based reachable tube contains the mixed reachable tube with at least a probability of $1-\alpha T$,
    \begin{align}
     \prob_{ \mathcal{D}}\Big[\mrt(S_0, T, \mathcal{D}) \subseteq \grt(S_0, T, \mathcal{D}) \Big] \geq 1-\alpha T,
\end{align}
\end{lemma}

% Then, I want to prove that:
% \begin{align}
%      \prob_{s \sim \mathcal{D}}\Big(\mrt(S_0, T) \subseteq \grt(S_0, T) \Big) \geq 1-\alpha,
% \end{align}

\textit{Proof of lemma \ref{lemma:mgtube-contain}.} Since we have already proven the first time-step reachable set containment in equation~\ref{eq: 1st-step}, we want to prove the second $\gamma$-based inflated reachable set contains the second $\gamma-\delta$ mixed reachable set with at least a probability of $1-\alpha$. To start with, we need to prove the second step $\gamma$-based control action set encompasses the $\gamma-\delta$ mixed control action set at the time $t=1$ with at least a probability of $1-\alpha$. The mixed $\gamma-\delta$ and $\gamma$-based control action set are described as below:

\begin{align}
    U_{m}^1 = \{u| s \in \grs(1, D_0) , u \in [\cld(s) - \delta(s), \cld(s) + \delta(s) ]  \} 
    \label{eq:Ut0mixed}
\end{align}
\begin{align}
    U_{\bar{\gamma}_{D_1}}^1 = \{u| s \in \grs(1, D_0), u \in [\cld(s) - \bar{\gamma}_{D_1}, \cld(s) + \bar{\gamma}_{D_1} ]    \} \label{eq:Ut0gamma}
\end{align}

Since the set for sampling states to calculate the $\bar{\gamma}$ is the same set to obtain the next mixed inflated reachable set, drawing from lemma~\ref{lemma:org-cp}, Definiton~\ref{def:exact-time-discrepancy},~\ref{def:time-variant-gamma}, and equation~\ref{eq:Ut0mixed},~\ref{eq:Ut0gamma} we conclude that,

\begin{align}
    \prob_{ D_{0:1} }[U_{m}^1 \subseteq U_{\bar{\gamma}_{D_1}}^1 ] \geq 1 - \alpha \label{eq:deltagammaU}
\end{align}

The next reachable set contains all the states starting from all the control actions within the control set. Therefore,
\begin{align} 
    \prob_{D_{0:1} }  \Big[ \mrs(2, D_{0}) \subseteq \grs(2, D_{0:1}) \Big] \geq 1-\alpha 
\end{align}

Following a similar procedure, for each time $t \in \{1, \cdots, T\}$ individually, this statement holds: 
\begin{align}
    \prob_{D_{0:t-1}}  \Big[ \mrs(t, D_{t-2}) \subseteq \grs(t, D_{t-1}) \Big] \geq 1-\alpha 
\end{align}

We take the opposite side of this statement,
\begin{align}
\prob_{D_{0:t-1}}  \Big[ \mrs(t, D_{t-2}) \supset \grs(t, D_{t-1}) \Big] < \alpha
\end{align}

Applying Boole's inequality gives us
\begin{align}
\prob_{D_{0:t-1}} \Big[ \exists t>0 \text{ s.t. } \mrs(t, D_{t-2}) \supset \grs(t, D_{t-1}) \Big] \leq \sum_{i=1}^T \alpha = \alpha T 
\end{align}

We finally conclude that,
\begin{align}
\prob_{D_{0:t-1}}  \Big[ \forall t \in \{1,..., T\} \text{ s.t. } \mrs(t, D_{t-2}) \subseteq \grs(t, D_{t-1}) \Big] \geq 1- \alpha T 
\end{align}

Therefore, we conclude that the $\gamma$-based inflated tube contains the $\gamma-\delta$ mixed reachable tube with at least a probability of $1-\alpha T$:
\begin{align}
\prob_{\mathcal{D}}  \Big[  \mrt(S_0, T, \mathcal{D}) \subseteq \grt(S_0, T, \mathcal{D}) \Big] \geq 1- \alpha T
\end{align}

The mixed $\gamma-\delta$ inflated reachable tube is an approximated high-dimensional reachable tube.
{\color{blue}{To do: Need to analyze the relationship between the mixed inflated reachable tube and the high-dimensional reachable tube}}


\subsection{Covariant shift for conformal prediction}

We aim to provide the confident action discrepancy for each reachable set at each time step. Based on the previous conformal prediction definition, we can apply the brute-force method that samples states following the uniform distribution over each reachable set to calculate the confidence bound. However, since the area and shape of each reachable set vary dramatically and are unpredictable, the brute-force method needs millions of points to sample, which is time-consuming and impractical. 

One type of distribution shift the conformal prediction can handle is \textit{covariant shift}. Assume we apply the distribution $D$ to sample points $\{X_i\}_{i=1}^{n}$ for training and calibration (calculate the CP values), covariant shift describes the situation where the distribution of the test data $\{X_i^{test}\}_{i=1}^{n}$ changes from $D$ to $D_{test}$. The covariant shift happens when we calculate the confidence interval over the reachable set. We sample points following the uniform distribution of whole state space $D_{all}$ for training and calibration. However, we need another uniform distribution over the reachable set $D_{sub}$ to get the corresponding confident bounds at each time step.

To solve the covariant shift, the weighted conformal prediction is put forward in the citation by assuming the likelihood of two distributions is known, namely $$\omega(x) = \frac{D_{test}(x)}{D(x)} $$ 

% This is usually the ratio of the new PDF to the old PDF.

Initially, we sample $n$ data points $\{X_i\}_{i=1}^{n}$ following the uniform distribution $D(x)$. Then we can define the weights, 
$$p_i^w(x) = \frac{\omega(X_i)}{\sum_{j=1}^{n}\omega(X_j) + \omega(x)}, i = 1, \dots, n, ~\text{and}~ p_{n+1}^w(x) = \frac{\omega(x)}{\sum_{j=1}^{n}\omega(X_j) + \omega(x)} $$
The $p_i^w(x)$ changes the probability for non-conformity scores by changing the probability of each sample $X_i$. Therefore, we can intuitively understand that the weights $p_i^w(x)$ are large when $X_i$ follow more on the new distribution; the $p_{n+1}^w(x)$ is large when input $x$ follows more on the new distribution; Therefore, these weights shift the probability of each non-conformity score. Assume we sample $\{x_i\}_{i=1}^n$ from the distribution $D$ and then we calculate the corresponding non-conformity scores $\{s_i\}_{i=1}^n$. Then we can express the conformal quantile in the new distribution $D_{test}$ as the $1-\alpha$ quantile of a reweighted distribution, 
$$\hat{q} = \inf \Bigl\{ s_j: \sum_{i = 1}^{j} p_i^w(x) \mathbf{1}\{s_i \leq s_j\} \geq 1 - \alpha \Bigl\}$$



\subsection{Discrepancy regression model}

Problem formulation: given a limited sampled dataset following one unknown distribution over the whole set (e.g., the robustness or our trajectory/action discrepancy), how can we obtain a set containing all the values in the given sub-region with a specified probability?



One potential solution is to apply conformal prediction over the whole region to get the statistical action/trajectory-based discrepancy that could be regarded as the corresponding discrepancy over any sub-region. One problem is that the distributions of the discrepancy over the whole space and the subspace could be different, leading to different confidence bounds. For example, If the distribution of the whole space is a zero-mean Gaussian distribution with 0.1 variances, and the distribution of one subspace is a zero-mean Gaussian distribution with 0.9 variances, the conformal prediction results on the whole space cannot be applied to the subspace. 

Another solution is to combine the regression model with the conformal prediction to eliminate the distribution problem above. First, a regression model mapping the relation between the states and discrepancy is trained over the whole space. With any open-loop verification tools, we can obtain the upper and lower bounds of the regression model over the whole region, namely $\mu_{min}, \mu_{max}$. With the help of Xin Qin's paper, these bounds will be inflated by conformal prediction such that $\text{P}(\forall x \in X_0, y(x) \in [\mu_{min} - d, \mu_{max} + d] ) \geq 1 - \alpha$. The bounds $[\mu_{min} - d, \mu_{max} + d]$ can be applied to represent bounds over any subsets within this whole region for several reasons: The upper and lower bounds of regression model over the whole space contain the upper and lower bounds over the subspace, namely $\forall S_i \subseteq S, i = 1, 2, \dots, n, [\mu_{min}^i, \mu_{max}^i] \subseteq [\mu_{min}, \mu_{max}]$. With the help of the regression model, we switch the discrepancy distribution problem to the distribution of residual $d$ between true discrepancy and the prediction of a regression model. The $d$ provides a confidence bound for every point sampled, i.i.d in the whole space, including the two points leading to the 
$u_{min}^i, u_{max}^i$. 

{\color{blue}Stop 03/11}

% How can we obtain this random variable's probability assurance (e.g., confidence interval) over given subsets of this whole set?

Two approaches involving conformal prediction are discussed: the first applies conformal prediction to calculate the confidence interval directly from the calibration dataset, and the second assesses the confidence discrepancy for a regression model. The necessity of the regression model is questioned, assuming that both methods applied to the same dataset denoted as $\mathcal{T} = \{ (\mathbf{x}_i, y_i) \}_{i=1}^{N}$ that is i.i.d. from set $X_0$. Each $\mathbf{x}_i$ represents $n$-dimension input, and each $y_i$ is the corresponding output.



Without using the regression model, the conformal prediction is directly applied to the dataset $\mathcal{T} = \{ (\mathbf{x}_i, y_i) \}_{i=1}^{N}$ with a specified error rate $\alpha$ to determine a confidence interval $m$. That ensures that $P( y_{N+1} < m) \geq 1 - \alpha$. 

When we consider applying a regression model to learn the underlying pattern of this set, we need to divide the overall data equally into a training set and a calibration set. The training set, $\mathcal{T}_{train} = \{ (\mathbf{x}_i, y_i) \}_{i=1}^{N/2}$, is used to train the regression model $\mu$, while the calibration dataset,  $\mathcal{T}_{cal} = \{ (\mathbf{x}_i, y_i) \}_{i=N/2+1}^{N}$, is used to calculate the confidence interval $d$ over the regression prediction such that $\text{P}( y_{n+1} \in [ \mu(x_{n+1}) - d, \mu(x_{n+1}) + d ] ) \geq 1 - \alpha$, where the $\alpha$ is the given error rate. The $d$ describes the confidence discrepancy between model prediction and the actual values. Given a trained regression model $\mu$ and the input set $X_0$, we can get the maximum and minimum value of the regression model within the specified input set, namely $\mu_{min}, \mu_{max}$. Therefore, we conclude that $\text{P}(\forall x \in X_0, \mu(x) \in [\mu_{min} - d, \mu_{max} + d] ) \geq 1 - \alpha$. Intuitively, this method provides the confidence interval over the upper and lower bounds instead of each point within this set, which is critical for safety verification problems.

The critical difference is that the first one can ensure that the $1-\alpha$ of the initial region will be safe due to the uniform distribution for sampling. In contrast, the second one ensures that the probability of the statement "all the region will be safe" is above $1 - \alpha$. The second method provides a stronger safety guarantee than the first one, especially in safety-critical problems. Considering a dataset of 100 points, 96 points are safe (robustness value above 0), and 4 points are unsafe (robustness value below 0). Given the error rate $\alpha = 5\%$, after merely applying the conformal prediction, we conclude that this region is safe with more than 95\% confidence. However, after training the regression model and calculating the confidence discrepancy, the value $\mu_{min} - d$ should be below zero, indicating unsafe in the same region. Considering the practical use, if we have already obtained some unsafe points within this set, there is no point in declaring this region is safe under 95\% confidence. Instead, we should declare that this region is unsafe with 100\%. The same conclusion fits our action-based and trajectory-based discrepancy. 

I put forward another conformal prediction method by providing confidence and assurance on whether the output of the next point will fall in the upper and lower bounds of this region. Given a calibration dataset and the upper and lower bound $[ \mu_{min}, \mu_{max}  ]$ of the trained regression model $\mu$ within the set $X_0$, we calculate the distance between each point in the calibration data and the upper and lower bound $[ \mu_{min}, \mu_{max}  ]$. The distance will be zero if the calibration point is within the bounds. Otherwise, the distance will be $\text{min}\{\|y_i - \mu_{min}\|, \|y_i - \mu_{max}\|\}$. By applying the conformal prediction, we obtain confidence bound $d_{bound}$ with specified error rate $\alpha$ such that $\operatorname{P}(\forall x \in X_0, \mu(x) \in [\mu_{min} - d_{bound}, \mu_{max} + d_{bound}]) \geq 1 - \alpha$.

Therefore, our problem transfers to which model can provide better upper and lower bounds on the discrepancy. The Gaussian process regression, polynomial estimation, and neural network regression can all provide the confidence interval. Then we can compare which model can achieve the highest precision value.

{\color{blue}New stop}


% Here are two different methods with conformal prediction: the first one is that we apply the calibration dataset to get the conformal prediction value, and the second one is that we provide the confidence difference over the regression model.   

% The first question is why we need the regression model. To begin with, I assume that the same dataset was applied to both methods. The overall dataset is denoted as $\mathcal{T} = \{ (\mathbf{x}_i, y_i) \}_{i=1}^{N}$ that is i.i.d. sampled from set $X_0$, where the $\mathbf{x}_i$ is the i-$th$ with $n$-dimension input and the $y_i$ is the corresponding i-$th$ output.

% We separate the overall data set evenly into two parts: the training dataset and the calibration dataset. The regression model $\mu$ was trained on training data, which is denoted as $\mathcal{T}_{train} = \{ (\mathbf{x}_i, y_i) \}_{i=1}^{N/2}$ and calculate the confidence discrepancy between the regression model $\mu$ and the ground truth on the calibration dataset (ground truth), namely $\mathcal{T}_{cal} = \{ (\mathbf{x}_i, y_i) \}_{i=N/2+1}^{N}$, where we apply conformal prediction to calculate the $d$ given error rate $\alpha$ such that $P( y_{N+1} \in [ \mu(x_{n+1}) - d, \mu(x_{n+1}) + d ] ) \geq 1 - \alpha$. The conformal prediction value $d$ depicts the confidence difference between the regression model and ground truth. Given a trained regression model $\mu$ and the input set $X_0$, we can get the maximum and minimum value of the regression model within the specified input set, namely $\mu_{min}, \mu_{max}$. Therefore, $\text{P}(\forall x \in X_0, y(x) \in [\mu_{min} - d, \mu_{max} + d] ) \geq 1 - \alpha$.

% When no regression model is involved, given $\mathcal{T} = \{ (\mathbf{x}_i, y_i) \}_{i=1}^{N}$, we apply conformal prediction on this dataset with error rate $\alpha$ to get the $m$ threshold, such that $P( y_{N+1} < m) \geq 1 - \alpha$.

% The second method has a more robust safety guarantee than the first one. Take one 100 training data example, where 96 points are safe (robustness value above 0), and 4 points (robustness value below 0) are unsafe. Given the error rate $\alpha = 5\%$, after only applying the conformal prediction without any regression models involved, we conclude that this region is safe with more than 95\% confidence. However, after training the regression model and calculating the difference, the $\mu_{min} - d$ should be below zero, indicating unsafe in the same region.


Obtaining the time-invariant action discrepancy $\bgamma$ is tricky because this involves sampling states following the same distribution over each inflated reachable set. It is infeasible due to millions of sampled points during the whole process. Instead, we put forward a regression model to describe the discrepancy over the whole state space and then provide the statistical upper bound for this regression model by conformal prediction. Here are two questions: 1. Does the lemma 3 hold? 

Can I improve the inverted pendulum CAV version? Using Neural Architect Search to obtain better LDC. Then, a regression model will be trained to describe the action-based and trajectory-based discrepancies. I can train 100 LDCs.

Don't forget the perception model. 

==> subsections/table_comp.tex <==
\begin{table}[ht!]
\centering
\caption{Summary of verification tools for neural-network controlled systems.}
\begin{tabular}[t]{l>{\raggedright}p{0.09\linewidth}>{\raggedright}p{0.14\linewidth}>{\raggedright}p{0.19\linewidth}>{\raggedright\arraybackslash}p{0.19\linewidth}}
\toprule
Name &Plant dynamics &Action space &Activation function &Core technique\\
\midrule
ReachNN*~\cite{reachnn} &Linear, Nonlinear & Discrete, Continuous &Relu, Sigmoid, Tanh &TM, Bernstein polynomial, parallel computation \\

POLAR~\cite{polar} &Linear, Nonlinear & Discrete, Continuous &Any non-differentiable function &TM, Bernstein polynomial, Symbolic reminder \\

Verisig~\cite{verisig} &Linear, Nonlinear & Discrete, Continuous &Sigmoid, Tanh &TM, hybrid-system-based \\

Sherlock~\cite{sherlock} &Linear, Nonlinear & Discrete, Continuous &Relu & TM, MILP \\

NNV~\cite{nnv} &Linear, Nonlinear & Discrete, Continuous &Relu, Sigmoid, Tanh &Star, zonotope, Abstract-domain \\
\bottomrule
\end{tabular}
\label{tab:relwork}
\end{table}
